Planck 2015 results. XIV. Dark energy and modified gravity

We study the implications of Planck data for models of dark energy (DE) and modified gravity (MG), beyond the cosmological constant scenario. We start with cases where the DE only directly affects the background evolution, considering Taylor expansions of the equation of state, principal component analysis and parameterizations related to the potential of a minimally coupled DE scalar field. When estimating the density of DE at early times, we significantly improve present constraints. We then move to general parameterizations of the DE or MG perturbations that encompass both effective field theories and the phenomenology of gravitational potentials in MG models. Lastly, we test a range of specific models, such as k-essence, f(R) theories and coupled DE. In addition to the latest Planck data, for our main analyses we use baryonic acoustic oscillations, type-Ia supernovae and local measurements of the Hubble constant. We further show the impact of measurements of the cosmological perturbations, such as redshift-space distortions and weak gravitational lensing. These additional probes are important tools for testing MG models and for breaking degeneracies that are still present in the combination of Planck and background data sets. All results that include only background parameterizations are in agreement with LCDM. When testing models that also change perturbations (even when the background is fixed to LCDM), some tensions appear in a few scenarios: the maximum one found is \sim 2 sigma for Planck TT+lowP when parameterizing observables related to the gravitational potentials with a chosen time dependence; the tension increases to at most 3 sigma when external data sets are included. It however disappears when including CMB lensing.

==> dark_energy_results.tex <==

%Results are shown in Fig.(\ref{fig:soundspeed})

%Interestingly, Planck alone would find a good model with low $c_s^2$ and $w \sim 0$. But when BAO is included w moves back to -1 and no strong constraint is found on $c_s^2$. Tests on-going to include ISW in the analysis and see if it breaks the degeneracy.

%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.3\textwidth]{figures/cs2w_2D_planck.pdf}
%%\includegraphics[width=0.3\textwidth]{figures/cs2w_2D_planck_BAO.pdf}
%\caption{Constraints on quintessence sound speed and w(z). (Using clik8.1, to be updated) Planck only.}
%\label{fig:soundspeed}
%\end{center}
%\end{figure*}

%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.4\textwidth]{figures/cs2w/compare_w_cs2w_2D.pdf}
%\includegraphics[width=0.4\textwidth]{figures/cs2w/compare_H0_cs2w_2D.pdf}
%\caption{Case $w$, $c_s^2$: constraints on quintessence sound speed and w(z) for different combinations of the datasets. To test whether including ISW breaks the degeneracy.}
%\label{fig:soundspeed}
%\end{center}
%\end{figure*}
\subsection{Dark energy sound speed}
\comment{What should we do with this? }
We consider a wCDM model, in which Dark Energy is characterized by a constant equation of state w and we allow the sound speed of Dark Energy $c_s^2$ to be different from 1, which is the value it would have in a minimal quintessence scalar field that does not contribute to clustering. We then vary both $w(z)$ and $c_s^2$. Results show that no constraint is found on the sound speed.

